On Using Chatbots to Promote Smoking Cessation Among Adolescents of Low Socioeconomic Status

Reducing youth tobacco use is critical for improving child health since tobacco use is associated with respiratory problems, and nicotine may interfere with healthy brain development. While tobacco regulation has contributed to declines in cigarette use among youth, these declines have occurred more quickly for youth of high socioeconomic status (SES) compared to youth of low SES. A major barrier to smoking cessation for adolescents of low SES is coordination of access and transportation to in-person treatment sessions. Low-SES youth may have family obligations that limit their ability to access in-person treatment. At the same time, mobile use among adolescents is high: 85% have smartphones. Additionally, adolescents engage in texting at high rates, suggesting that they are well-suited for mobile instant messaging interventions. Mobile interventions have shown promise for youth, but their use remains low. Thus, more research is needed to develop effective and engaging mobile interventions to increase quit rates. In this paper, we provide a brief review of approaches to adolescent smoking cessation and describe the promise of chatbots for smoking cessation.

==> table/auto_eval.tex <==
\begin{comment}

\begin{table}[htbp]
\tiny
\begin{tabular}{@{}llllllll@{}}
              & BLEU\_1 & BLEU\_2 & BLEU\_3 & BLEU\_4 & METEOR & ROUGE\_L & CIDEr \\ \midrule
GLAC      & .374   & .185   & .093   & .050   & .297  & .250    & .049 \\
No KG        & .376   & .185   & .096   & .050   & .295  & .237    & .055 \\
OpenIE        & .446   & .223   & .109   & .056   & .297  & .241    & .094 \\
VisualGenome & .451   & .223   & .109   & .056   & .296  & .241    & .096 \\ \bottomrule
\end{tabular}
\caption{\small Comparison for four models on seven kinds of automatic evaluation.}
\end{table}

\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htbp]
\resizebox{1\columnwidth}{!}{
\begin{tabular}{@{}lrrrrr@{}}
\toprule
 & \textbf{BLEU1} & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{CIDEr} \\ \midrule
\textbf{GLAC~\cite{Kim2018GLACNG}} & .374 & .050 & \textbf{.297} & \textbf{.250} & .049 \\ \midrule
\textbf{No KG} & .376 & .050 & .295 & .237 & .055 \\
\textbf{OpenIE} & .446 & \textbf{.056} & \textbf{.297} & .241 & .094 \\
\textbf{Visual Genome} & \textbf{.451} & \textbf{.056} & .296 & .241 & \textbf{.096} \\ \bottomrule
\end{tabular}
}
\caption{Automatic evaluation results. Prior work has clearly shown that the classic automatic evaluation metrics are
weak or even negative quality indicators for visual 
storytelling~\cite{hsu-etal-2019-visual,wang2018nometics}.}
\label{tab:auto_eval}
\end{table}



==> table/coreference.tex <==
\begin{table}[]
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l|l|l}
 &\includegraphics[width=0.17\textwidth]{figure/dog1.jpg}
 &\includegraphics[width=0.17\textwidth]{figure/dog2.jpg} \\ \hline
\begin{tabular}[c]{@{}l@{}}Original \\ story\end{tabular} & \begin{tabular}[c]{@{}l@{}}The dog is\\  ready to go.\end{tabular} & \begin{tabular}[c]{@{}l@{}}He is playing \\ on the ground.\end{tabular}      \\ \hline
Terms                                                     & \begin{tabular}[c]{@{}l@{}}``Dog\_Noun'',\\  ``Motion\_Frame''\end{tabular}             & \begin{tabular}[c]{@{}l@{}}``Performers\_and\_roles\_Frame'',\\ ``Ground\_Noun''\end{tabular}                   \\ \hline\hline
\begin{tabular}[c]{@{}l@{}}Story \\ w/ CR\end{tabular}    & \begin{tabular}[c]{@{}l@{}}The dog is \\ ready to go.\end{tabular} & \begin{tabular}[c]{@{}l@{}}The dog is playing \\ on the ground.\end{tabular} \\ \hline 
Terms                                                     & \begin{tabular}[c]{@{}l@{}}``Dog\_Noun'',\\ ``Motion\_Frame''\end{tabular}             & \begin{tabular}[c]{@{}l@{}}``Dog\_Noun'',\\ ``Performers\_and\_roles\_Frame'',\\  ``Ground\_Noun''\end{tabular}           \\ \hline
\end{tabular}
}
\caption{Term extraction and coreference replacement (CR). Image
order is from left to right.}
\label{tab:term_example}
\end{table}


==> table/error_analysis.tex <==
\begin{table}[]
\begin{tabular}{l|l}
                             & Story \\ \hline
Grounded Error               & 22    \\
Relation Error               & 13    \\
Model Story Generation Error & 15  
\label{tab:error_analysis_1}
\end{tabular}
\end{table}

\begin{table}[]
\begin{tabular}{ll}
        & Grounded Error                                                                                                                                                                 \\ \hline
Example & OpenIE: we went to a museum today . the room was very old . we had a great time there . the band went on for a long time . the band played music . then we came back to town . \\
Cons    & There is no museum in the images                                                                                                                                     \label{tab:error_analysis_2}
\end{tabular}
\end{table}

\begin{table}[]
\begin{tabular}{ll}
        & Relation Error                                                                                                                                                                 \\ \hline
Visual Genome: i went to the city today . there were many people gathered to watch . when i got there they looked like a zebra food . it was a lot of good food . everyone had a great time . the crowd was very big .\\
Cons    & The object generated by Visual Genome: zebra is not in the images.                                                                                             \label{tab:error_analysis_3}
\end{tabular}
\end{table}

\begin{table}[]
\begin{tabular}{ll}
        & Model Story Generation Error                                                                                                                                                                 \\ \hline
17398173-17399304-17399712-17400033-17401748-
Visual Genome: the family got together for dinner . the food was very tasty . we put some food in a napkin as well . the main dish was delicious . we ate it all . we had a lot of drinks .\\
Cons    & The images are related to restaurant, so it's reasonable to have napkins in the term set.  However, the model generates "we put some food in a napkin as well", which use the napkins to construct an inappropriate sentence.                                                                                             \label{tab:error_analysis_3}
\end{tabular}
\end{table}

==> table/standard_comparison.tex <==
\begin{table}[!ht]
\centering
\small
%\resizebox{0.8\textwidth}{!}{
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
%Team & Focused & Coherent & Shareable & Human & Grounded & Detailed & Entertaining  \\
 & F & C & S & H & G & D   \\
\midrule
Human & 3.64 & 3.47 & 3.19 & 3.45 & 3.59 & 3.49 \\
\midrule
SnuBiVtt & 3.18	& 3.00	& 2.82	& 2.86	& 2.78	& 2.80  \\
\midrule\midrule

Enhanced PlotVist\\
\midrule
%\begin{tabular}[c]{@{}l@{}}$\text{PlotVIST}^{\text{1+}}$\end{tabular}
\begin{tabular}[c]{@{}l@{}}$\hspace{3mm}\text{-w/o KB}$\end{tabular}
& \textbf{3.22} & \textbf{3.24} & \textbf{3.21} & \textbf{3.27} & 3.25 & 3.24  \\

\begin{tabular}[c]{@{}l@{}}$\hspace{3mm}\text{-w/ KB: random}$\end{tabular} & 3.08 & 3.14 & 3.15 & 3.16 & \textbf{3.28} & \textbf{3.30} \\

\begin{tabular}[c]{@{}l@{}}$\hspace{3mm}\text{-w/ KB: scoring}$\end{tabular} & 3.21 & 3.13 & 3.11 & 3.13 & 3.12 & 3.11 \\ 
\midrule


\end{tabular}
}

\caption{\small Standard rating evaluation for Improved \system for six categories:
\focus (F), \coherence (C), \shareability (S), \humanness (H), \grounding (G), and \detail (D).}

\label{tab:emnlp-standard}

\end{table}


==> table/with_or_without_image_comparison_table.tex <==



% \begin{table}[!ht]
% \centering
% \small
% \resizebox{1\columnwidth}{!}{

% \begin{tabular}{ccccc}
% \toprule
%   & Human & SnuBiVtt & Basic PlotVist & $\text{PlotVist}^{\text{ w/o KB}}$ \\
%   %& $\text{P}^{\text{2+}}$ \\
% \midrule
% Overall & 2.04 & 3.18 & 3.34 & 3.28 \\
% %& \textbf{3.16}  \\
% % \midrule
% % Entertaining & 2.20 & 3.21 & 3.41 & 3.13 & \textbf{3.06} \\
% \midrule
% $\text{Overall}^-$ & 2.15 & \textbf{2.76} & 3.34 & 3.34 \\
% %& 3.41 \\
% \midrule 

% \end{tabular}
% }

% \caption{\small Direct comparison evaluation for the basic \system model. Numbers indicate average rank given to stories (from 1 to 5, lower is better).}
% \label{tab:comp_result_basic}

% \end{table}


\begin{table}[!ht]
\centering
\small
\resizebox{1\columnwidth}{!}{


\begin{tabular}{cccccc}
\toprule
  & Human & SnuBiVtt & $\text{P}^{\text{ w/o KB}}$ & $\text{P}^{\text{ random}}$ & $\text{P}^{\text{ scoring}}$ \\
\midrule
Overall & 2.42 & 3.16 & 3.42 & 3.02 & \textbf{2.98}  \\
% \midrule
% Entertaining & 2.33 & 3.19 & 3.46 & 3.02 & \textbf{3.00} \\
\midrule
$\text{Overall}^-$ & 2.55 & \textbf{2.98} & 3.32 & 3.11 & 3.04 \\
\midrule 

\end{tabular}
}

\caption{\small Direct comparison evaluation for the enhanced \system model.
Numbers indicate average rank given to stories (from 1 to 5, lower is better).}
\label{tab:comp_result_improved}

\end{table}


